C-Learning: Horizon-Aware Cumulative Accessibility Estimation

Multi-goal reaching is an important problem in reinforcement learning needed to achieve algorithmic generalization. Despite recent advances in this field, current algorithms suffer from three major challenges: high sample complexity, learning only a single way of reaching the goals, and difficulties in solving complex motion planning tasks. In order to address these limitations, we introduce the concept of cumulative accessibility functions, which measure the reachability of a goal from a given state within a specified horizon. We show that these functions obey a recurrence relation, which enables learning from offline interactions. We also prove that optimal cumulative accessibility functions are monotonic in the planning horizon. Additionally, our method can trade off speed and reliability in goal-reaching by suggesting multiple paths to a single goal depending on the provided horizon. We evaluate our approach on a set of multi-goal discrete and continuous control tasks. We show that our method outperforms state-of-the-art goal-reaching algorithms in success rate, sample complexity, and path optimality. Our code is available at https://github.com/layer6ai-labs/CAE, and additional visualizations can be found at https://sites.google.com/view/learning-cae/.

==> ac_learning_paper_ICLR(2)/0-math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{mathtools}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ac_learning_paper_ICLR(2)/1-intro.tex <==
\section{Introduction}

% High level explanation for the changes I made to the intro: the previous version focus to some degree on talking about goal reaching in general.  I wanted to shift the focus to what the current methods are lacking and a high-level view of how we address that and what our contributions are.

%In a typical reinforcement learning (RL) setting an agent is trained to maximize the expected discounted return of some reward function. With the advent of neural networks, this framework has achieved remarkable successes in recent years \citep{mnih2015human, silver2016mastering}. This approach, however, lacks flexibility. Designing an adequate reward can be a difficult environment-specific challenge, and even in the presence of such a reward, the exact task which we wish the agent to perform may not be known at training time. We might instead wish to train a single agent equipped with the ability to reach one of several \emph{goals}, of which we select one per episode at test time.

Multi-goal reinforcement learning tackles the challenging problem of reaching multiple goals, and as a result, is an ideal framework for real-world agents that solve a diverse set of tasks. Despite progress in this field \citep{Kaelbling1993, schaul2015universal, andrychowicz2017hindsight, Ghosh2019}, current algorithms suffer from a set of limitations: an inability to find multiple paths to a goal,  high sample complexity, and poor results in complex motion planning tasks. In this paper we propose $C$-learning, a method which addresses all of these shortcomings.

%We address these challenges by proposing \textit{cumulative accessibility functions} $C(s,a,g,h)$, which correspond to the probability of reaching a goal $g$ from a given state $s$ within a specified horizon $h$. 

% Multi-goal agents have been studied previously. \citet{schaul2015universal} introduced Universal Value Function Approximators (UVFAs), which generalizes the  traditional value function to multiple goals. \citet{andrychowicz2017hindsight} proposed Hindsight Experience Replay (HER), which relabels the past experience by the achieved goals, and allows sample efficient learning from sparse rewards. In this paper, we solve the problem of multi-goal reinforcement learning with sparse rewards. We incorporate recent techniques, such as HER into our work for better performance. 

Many multi-goal reinforcement learning algorithms are limited by learning only a single policy $\pi(a|s, g)$ over actions $a$ to reach goal $g$ from state $s$. There is an unexplored trade-off between reaching the goal reliably and reaching it quickly. We illustrate this shortcoming in Figure \ref{fig:illustration_predator}, which represents an environment where an agent must reach a goal on the opposite side of some predator. Shorter paths can reach the goal faster at the cost of a higher probability of being eaten. Existing algorithms do not allow a dynamic choice of whether to act safely or quickly at test time.

The second limitation is sample complexity. Despite significant improvements \citep{andrychowicz2017hindsight, Ghosh2019}, multi-goal reaching still requires a very large amount of environment interactions for effective learning. We argue that the optimal $Q$-function must be learned to high accuracy for the agent to achieve reasonable performance, and this leads to sample inefficiency. The same drawback of optimal $Q$-functions often causes agents to learn sub-optimal ways of reaching the intended goal. This issue is particularly true for motion planning tasks \citep{motionplanning}, where current algorithms struggle. 

We propose to address these limitations by learning horizon-aware policies $\pi(a|s,g,h)$, which should be followed to reach goal $g$ from state $s$ in at most $h$ steps. The introduction of a time horizon $h$ naturally allows us to tune the speed/reliability trade-off, as an agent wishing to reach the goal faster should select a policy with a suitably small $h$ value. To learn these policies, we introduce the \textit{optimal cumulative accessibility function} $C^*(s,a,g,h)$. This is a generalization of the state-action value function and corresponds to the probability of reaching goal $g$ from state $s$ after at most $h$ steps if action $a$ is taken, and the agent acts optimally thereafter. Intuitively it is similar to the optimal $Q$-function, but $Q$-functions rarely correspond to probabilities, whereas the $C^*$-function does so by construction. 
% We derive Bellman backup update rules for $C^*$, which allow it to be learned, deriving a method we call cumulative accessibility estimation, or \emph{C-learning}.
We derive Bellman backup update rules for $C^*$, which allow it to be learned via minimization of unbiased estimates of the cross-entropy loss -- this is in contrast to $Q$-learning, which optimizes biased estimates of the squared error. Policies $\pi(a|s,g,h)$ can then be recovered from the $C^*$ function.
We call our method cumulative accessibility estimation, or \emph{C-learning}. \citet{pong2018temporal} proposed TDMs, a method involving horizon-aware policies. We point out that their method is roughly related to a non-cumulative version of ours with a different loss that does not enable the speed/reliability trade-off and is ill-suited for sparse rewards. We include a detailed discussion of TDMs in section \ref{sec:c_learning}.

One might expect that adding an extra dimension to the learning task, namely $h$, would increase the difficulty - as $C^*$ effectively contains the information of several optimal $Q$-functions for different discount factors. However, we argue that $C^*$ does not need to be learned to the same degree of accuracy as the optimal $Q$-function for the agent to solve the task. As a result, learning $C^*$ is more efficient, and converges in fewer environmental interactions. This property, combined with our proposed goal sampling technique and replay buffer used during training, provides empirical improvements over $Q$-function based methods.

%This is a surprising fact, as one could naively expect learning to become harder by adding a variable, namely $h$, to the problem. 

In addition to these advantages, learning $C^*$ is itself useful, containing information that the horizon-aware policies do not. It estimates whether a goal $g$ is reachable from the current state $s$ within $h$ steps. In contrast, $\pi(a|s,g,h)$ simply returns some action, even for unreachable goals. We show that $C^*$ can be used to determine reachability with examples in a nonholonomic environment.

%This naturally lends itself to incorporation into other frameworks, for example, in goal setting for hierarchical RL tasks \citep{nachum2018data}, or safety-critical environments requiring adaptation \citep{peng2018sim, zhang2020carl}.

%We also explore the motion planning problem with multi-goal reinforcement learning. An ideal motion planner finds the optimal path between two states in real-time. Despite recent advances in reinforcement learning, RL algorithms have not yet been fully deployed in motion planning tasks due to insufficient performance \citep{motionplanning}.
%However, our method naturally learns the optimal path by computing reachability of the goal for different horizons and defining the policy based on the smallest reachable horizon.

%Additionally, we are improving sample complexity by incorporating environment dynamics -- as in model-based RL algorithms, which are known to learn with fewer samples \textbf{CITE} -- into our method in the short-horizon case. 
%Model-based RL algorithms tend to learn with fewer samples by learning the environments dynamics. 
%In our algorithm, estimated environment dynamics will be included into $C$ function as a special case of $C(s,a,g,h=1)$. 

% The following is a summary of our major contributions: 

% \begin{itemize}
% \item Introducing $C^*$-functions and cumulative accessibility estimation. We derive Bellman backup update rules that allow learning from offline interactions. We study these functions and prove $C^*$ is non-decreasing in horizon.

% \item By visualizing the reachability results, we demonstrate that $C^*$-functions can learn the environment's underlying reachability.

% \item Using the $C^*$-function, we derive a learning algorithm for both discrete and continuous action spaces and demonstrate our method outperforms current state-of-the-art RL algorithms.

% \item We evaluate our method on complex motion planning environments and show our method outperforms other RL algorithms in finding the optimal path.

% \item We extend our method to stochastic environments. As discussed in \citet{multigoal}, HER relabeling can result in bias in stochastic environments. To address this issue, we propose a novel relabeling method. We perform experiments on the frozen lake environment and demonstrate that the user can tune speed/reliability trade-off by specifying the horizon in the policy.  
% \end{itemize}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figures/mouse_cat-v2.png}
        %\caption{A continuous spectrum of paths allow the mouse to reach its goal faster, at an increased risk of disturbing the cat and being eaten.}
        \caption{}
        \label{fig:illustration_predator}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=0.6\textwidth]{figures/accuracy_illustration.png}
        \caption{}
        \label{fig:q_accuracy}
    \end{subfigure}
    \caption{$(a)$ A continuous spectrum of paths allow the mouse to reach its goal faster, at an increased risk of disturbing the cat and being eaten. $(b)$  $Q^*$ (with $\gamma = 0.99$) needs to be learned more accurately than $C^*$ to act optimally. The goal $g$ can be reached in $h^*=5$ steps from $s$, so that $Q^*(s, g, a^*) = 0.99^5$ and $Q^*(s, g, a_-) = 0.99^7$; while $C^*(s, a^*, g, h^*) = 1$ and $C^*(s, a_-, g, h^*) = 0$.}
\end{figure}

\textbf{Summary of contributions}: $(i)$ introducing $C$-functions and cumulative accessibility estimation for both discrete and continuous action spaces; $(ii)$ highlighting the importance of the speed vs reliability trade-off in finite horizon reinforcement learning; $(iii)$ introducing a novel replay buffer specially tailored for learning $C^*$ which builds on HER \citep{andrychowicz2017hindsight}; and $(iv)$ empirically showing the effectiveness of our method for goal-reaching as compared to existing alternatives, particularly in the context of complex motion planning tasks.



==> ac_learning_paper_ICLR(2)/2-rel-work.tex <==

\section{Background and related work}\label{sec:background}

Let us extend the Markov Decision Process (MDP) formalism \citep{sutton1998introduction} for goal-reaching. We consider a set of actions $\mathcal{A}$, a state space $\mathcal{S}$, and a goal set $\mathcal{G}$. We assume access to a goal checking function $G: \mathcal{S} \times \mathcal{G} \rightarrow \{0, 1\}$ such that $G(s, g)=1$ if and only if state $s$ achieves goal $g$. For example, achieving the goal could mean exactly reaching a certain state, in which case $\mathcal{G}=\mathcal{S}$ and $G(s, g)=\mathds{1}(s=g)$.
For many continuous state-spaces, hitting a state exactly has zero probability.
Here we can still take $\mathcal{G} = \mathcal{S}$, but let $G(s, g)=\mathds{1}(d(s,g)\leq \epsilon)$ for some radius $\epsilon$ and metric $d$.
More general choices are possible.
For example, in the Dubins' Car environment which we describe in more detail later, the state consists of both the location and orientation of the car: $\mathcal{S} = \mathbb{R}^2 \times S^1$.
We take $\mathcal{G} = \mathbb{R}^2$, and $G(s, g)$ checks that the location of the car is within some small radius of $g$, ignoring the direction entirely.
For a fixed $g$, $G(s, g)$ can be thought of as a sparse reward function.

In the goal-reaching setting, a policy $\pi: \mathcal{S} \times \mathcal{G} \rightarrow \mathcal{P}(\mathcal{A})$, where $\mathcal{P}(\mathcal{A})$ denotes the set of distributions over $\mathcal{A}$, maps state-goal pairs to an action distribution. The environment dynamics are given by a starting distribution $p(s_0, g)$, usually taken as $p(s_0)p(g)$, and transition probabilities $p(s_{t+1}|s_t, a_t)$. States for which $G(s, g) = 1$ are considered terminal.

%\textbf{Q-Learning:}  \citet{schaul2015universal} has extended $Q$-function \citep{watkins1992q} to the multi-goal reaching setting. $Q^\pi:\mathcal{S} \times \mathcal{G} \times \mathcal{A} \rightarrow \mathbb{R}$ is defined by $Q^\pi(s_t, g, a_t) = \mathbb{E}_\pi[\sum_{i=t}^\infty \gamma^{i-t} G(s_t, g)|s_t, a_t]$, where $\gamma \in [0,1]$ is a discount factor and the expectation is with respect to state-action trajectories obtained by using $\pi(a|s_i, g)$. If $\pi^*$ is an optimal policy in the sense that $Q^{\pi^*}(s, g, a) \geq Q^\pi(s, g, a)$ for every $\pi$ and $(s, g, a) \in \mathcal{S} \times \mathcal{G} \times \mathcal{A}$, then $Q^{\pi^*}$ matches the optimal $Q$-function, $Q^*$, which obeys the Bellman equation:
\textbf{Q-Learning:}  A $Q$-function \citep{watkins1992q} for multi-goal reaching, $Q^\pi:\mathcal{S} \times \mathcal{G} \times \mathcal{A} \rightarrow \mathbb{R}$, is defined by $Q^\pi(s_t, g, a_t) = \mathbb{E}_\pi[\sum_{i=t}^\infty \gamma^{i-t} G(s_t, g)|s_t, a_t]$, where $\gamma \in [0,1]$ is a discount factor and the expectation is with respect to state-action trajectories obtained by using $\pi(a|s_i, g)$. If $\pi^*$ is an optimal policy in the sense that $Q^{\pi^*}(s, g, a) \geq Q^\pi(s, g, a)$ for every $\pi$ and $(s, g, a) \in \mathcal{S} \times \mathcal{G} \times \mathcal{A}$, then $Q^{\pi^*}$ matches the optimal $Q$-function, $Q^*$, which obeys the Bellman equation:
\begin{equation}\label{eq:q_learning}
Q^*(s, g, a) = \mathbb{E}_{s' \sim p(\cdot|s, a)}\left[G(s, g) + \gamma \max_{a' \in \mathcal{A}} Q^*(s', g, a')\right].
\end{equation}
In deep $Q$-learning \citep{mnih2015human}, $Q^*$ is parameterized with a neural network and learning is achieved by enforcing the relationship from equation \ref{eq:q_learning}. This is done by minimizing $\sum_i \mathcal{L}(Q^*(s_i,g_i,a_i), y_i)$, where $y_i$ corresponds to the expectation in equation \ref{eq:q_learning} and is estimated using a replay buffer of stored tuples $(s_i, a_i, g_i, s_i')$. Note that $s'_i$ is the state the environment transitioned to after taking action $a_i$ from state $s_i$, and determines the value of $y_i$. Typically $\mathcal{L}$ is chosen as a squared error loss, and the dependency of $y_i$ on $Q^*$ is ignored for backpropagation in order to stabilize training. Once $Q^*$ is learned, the optimal policy is recovered by $\pi^*(a|s, g) = \mathds{1}(a=\argmax_{a'}Q^*(s,g,a'))$.

There is ample work extending and improving upon deep $Q$-learning \citep{haarnoja2018soft}. For example, \citet{lillicrap2015continuous} extend it to the continuous action space setting, and \citet{fujimoto2018addressing} further stabilize training. These improvements are fully compatible with goal-reaching \citep{pong2019skew, bharadhwaj2020leaf, Ghosh2019}.  \citet{andrychowicz2017hindsight} proposed Hindsight Experience Replay (HER), which relabels past experience as achieved goals, and allows sample efficient learning from sparse rewards \citep{nachum2018data}.




==> ac_learning_paper_ICLR(2)/3-c-functions.tex <==
\section{Cumulative accessibility functions}\label{sec:c_learning}

\begin{figure}[!t]
    \centering
    %\vspace{-10cm}
    \begin{minipage}[b]{.44\linewidth}
    \centering
    \resizebox{\textwidth}{!}{  
  \begin{tikzpicture}
    \node[shape=circle,draw=black, fill=gray!25, minimum size=11mm] (a) at (0,1) {\tiny$a$};
    \node[shape=circle,draw=black, minimum size=11mm] (a1) at (2,1) {\tiny$a_1$};
    \node[shape=circle,draw=black, minimum size=11mm] (a2) at (4,1) {\tiny$a_2$};
    \node[shape=circle,draw=black, minimum size=11mm] (a3) at (6,1) {\tiny$a_3$};
    
    \node[shape=circle,draw=black, fill=gray!25, minimum size=11mm , align=center] (s) at (-1,0) {\tiny $s$ \\ \tiny$h$};
    \node[shape=circle,draw=black, align=center, minimum size=11mm, path picture={\fill[gray!25] (path picture bounding box.east) rectangle (path picture bounding box.south west);}] (s1) at (1,0) {\tiny $s_1$\\ \tiny $h-1$};
    \node[shape=circle,draw=black, align=center, minimum size=11mm, path picture={\fill[gray!25] (path picture bounding box.east) rectangle (path picture bounding box.south west);}] (s2) at (3,0) {\tiny $s_2$\\ \tiny$h-2$};
    \node[shape=circle,draw=black, align=center, minimum size=11mm, path picture={\fill[gray!25] (path picture bounding box.east) rectangle (path picture bounding box.south west);}] (s3) at (5,0) {\tiny $s_3$\\ \tiny $h-3$};
    
    \node[shape=circle,draw=black, fill=gray!25, minimum size=11mm] (g) at (3,2) {\tiny$g$};
    
    \node[] () at (7,1) {\dots};
    \node[] () at (6,0) {\dots};
    
    
    \path [->] (a) edge node[left] {} (s1);
    \path [->] (a1) edge node[left] {} (s2);
    \path [->] (a2) edge node[left] {} (s3);

    \path [->] (s) edge node[left] {} (s1);
    \path [->] (s1) edge node[left] {} (s2);
    \path [->] (s2) edge node[left] {} (s3);
    
    \path [->] (s1) edge node[left] {} (a1);
    \path [->] (s2) edge node[left] {} (a2);
    \path [->] (s3) edge node[left] {} (a3);
    
    \path [->] (g) edge node[left] {} (a1);
    \path [->] (g) edge node[left] {} (a2);
    \path [->] (g) edge node[left] {} (a3);

\end{tikzpicture}
}
  \end{minipage}
  \begin{minipage}[b]{.55\linewidth}
  \centering
  \caption{Graphical model depicting trajectories from $\mathbb{P}_{\pi(\cdot|\cdot, g, h)}(\cdot|s_0=s, a_0=a)$. Gray nodes denote fixed values, and white nodes stochastic ones. Nodes $a$, $g$ and $s$ are non-stochastic simply because they are conditioned on, not because they are always fixed within the environment. Note that the values of $h$ decrease deterministically. Nodes corresponding to horizons could be separated from states, but are not for a more concise graph.}
    \label{fig:graph_model}
    %\vspace{-0.2cm}
    %\label{fig:toytest}
    \end{minipage}
\end{figure}


% \begin{wrapfigure}{0.5\textwidth}
%     \centering
%     \resizebox{0.5\textwidth}{!}{  
%   \begin{tikzpicture}
%     \node[shape=circle,draw=black, fill=gray!25, minimum size=11mm] (a) at (0,1) {\tiny$a$};
%     \node[shape=circle,draw=black, minimum size=11mm] (a1) at (2,1) {\tiny$a_1$};
%     \node[shape=circle,draw=black, minimum size=11mm] (a2) at (4,1) {\tiny$a_2$};
%     \node[shape=circle,draw=black, minimum size=11mm] (a3) at (6,1) {\tiny$a_3$};
    
%     \node[shape=circle,draw=black, fill=gray!25, minimum size=11mm , align=center] (s) at (-1,0) {\tiny $s$ \\ \tiny$h$};
%     \node[shape=circle,draw=black, align=center, minimum size=11mm, path picture={\fill[gray!25] (path picture bounding box.east) rectangle (path picture bounding box.south west);}] (s1) at (1,0) {\tiny $s_1$\\ \tiny $h-1$};
%     \node[shape=circle,draw=black, align=center, minimum size=11mm, path picture={\fill[gray!25] (path picture bounding box.east) rectangle (path picture bounding box.south west);}] (s2) at (3,0) {\tiny $s_2$\\ \tiny$h-2$};
%     \node[shape=circle,draw=black, align=center, minimum size=11mm, path picture={\fill[gray!25] (path picture bounding box.east) rectangle (path picture bounding box.south west);}] (s3) at (5,0) {\tiny $s_3$\\ \tiny $h-3$};
    
%     \node[shape=circle,draw=black, fill=gray!25, minimum size=11mm] (g) at (3,2) {\tiny$g$};
    
%     \node[] () at (7,1) {\dots};
%     \node[] () at (6,0) {\dots};
    
    
%     \path [->] (a) edge node[left] {} (s1);
%     \path [->] (a1) edge node[left] {} (s2);
%     \path [->] (a2) edge node[left] {} (s3);

%     \path [->] (s) edge node[left] {} (s1);
%     \path [->] (s1) edge node[left] {} (s2);
%     \path [->] (s2) edge node[left] {} (s3);
    
%     \path [->] (s1) edge node[left] {} (a1);
%     \path [->] (s2) edge node[left] {} (a2);
%     \path [->] (s3) edge node[left] {} (a3);
    
%     \path [->] (g) edge node[left] {} (a1);
%     \path [->] (g) edge node[left] {} (a2);
%     \path [->] (g) edge node[left] {} (a3);

% \end{tikzpicture}
% }
%  \caption{Graphical model depicting trajectories from $\mathbb{P}_{\pi(\cdot|\cdot, g, h)}(\cdot|s_0=s, a_0=a)$. Gray nodes denote fixed values, and white nodes stochastic ones. Nodes $a$, $g$ and $s$ are non-stochastic simply because they are conditioned on, not because they are always fixed within the environment. Note that the values of $h$ decrease deterministically. Nodes corresponding to horizons could be separated from states, but are not for a more concise graph.}
%     \label{fig:graph_model}
% \end{wrapfigure}



We now consider horizon-aware policies $\pi: \mathcal{S} \times \mathcal{G} \times \mathbb{N} \rightarrow \mathcal{P}(\mathcal{A})$, and define the cumulative accessibility function  $C^\pi(s,a,g,h)$, or $C$-function, as the probability of reaching goal $g$ from state $s$ in at most $h$ steps by taking action $a$ and following the policy $\pi$ thereafter.
By ``following the policy $\pi$ thereafter'' we mean that after $a$, the next action $a_1$ is sampled from $\pi(\cdot |s_1, g, h-1)$, $a_2$ is sampled from $\pi(\cdot |s_2, g, h-2)$ and so on.
See Figure \ref{fig:graph_model} for a graphical model depiction of how these trajectories are obtained. Importantly, an agent need not always act the same way at a particular state in order to reach a particular goal, thanks to horizon-awareness. We use $\mathbb{P}_{\pi(\cdot|\cdot,g,h)}(\cdot|s_0=s, a_0=a)$ to denote probabilities in which actions are drawn in this manner and transitions are drawn according to the environment $p(s_{t+1}|s_t, a)$. More formally, $C^\pi$ is given by:
\begin{equation}\label{eq:c_learning}
C^\pi(s,a,g,h) = \mathbb{P}_{\pi(\cdot|\cdot,g,h)}\left(\displaystyle \max_{t=0,\dots,h} G(s_t, g) = 1 \middle| s_0 = s, a_0 = a\right).
\end{equation}

\textbf{Proposition 1}: $C^\pi$ can be framed as a $Q$-function within the MDP formalism, and if $\pi^*$ is optimal in the sense that $C^{\pi^*}(s,a,g,h) \geq C^\pi(s, a, g, h)$ for every $\pi$ and $(s,a,g,h) \in \mathcal{S} \times \mathcal{A} \times \mathcal{G} \times \mathbb{N}$, then $C^{\pi^*}$ matches the optimal $C$-function, $C^*$, which obeys the following equation:
\begin{equation}\label{eq:c_learning_opt}
C^*(s,a,g,h) =
\begin{cases}
\mathbb{E}_{s' \sim p(\cdot|s,a)}\left[\displaystyle \max_{a' \in \mathcal{A}} C^*(s', a', g, h-1)\right] \text{ if }G(s, g)=0\text{ and }h \geq 1,\\
G(s, g)\hspace{127pt} \text{ otherwise} .
\end{cases}
\end{equation}
%\begin{proof}
See appendix \ref{sec:apprendix_proofs} for a detailed mathematical proof of this proposition. The proof proceeds by first deriving a recurrence relationship that holds for any $C^\pi$. In an analogous manner to the Bellman equation in $Q$-learning, this recurrence involves an expectation over $\pi(\cdot|s', g, h-1)$, which, when replaced by a $\max$ returns the recursion for $C^*$.
%\end{proof}

Proposition 1 is relevant as it allows us to learn $C^*$, enabling goal-reaching policies to be recovered:
\begin{equation}\label{eq:c_policy}
\pi^*(a | s, g, h) = \mathds{1}\left(a = \argmax_{a'}C^*(s, a', g, h)\right).
\end{equation}
$C^*$ itself is useful for determining reachability. After maximizing over actions, it estimates whether a given goal is reachable from a state within some horizon. Comparing these probabilities for different horizons allows us to make a speed / reliability trade-off for reaching goals.

% Second,
We observe that an \emph{optimal} $C^*$-function is non-decreasing in $h$, but this does not necessarily hold for \emph{non-optimal} $C$-functions. 
%We note that this statement is not true in general for non-optimal $C$-functions.
For example, a horizon-aware policy could actively try to avoid the goal for high values of $h$, and the $C^\pi$-function constructed from it would show lower probabilities of success for larger $h$. See appendix \ref{sec:apprendix_proofs} for a concrete example of this counter-intuitive behavior.

\textbf{Proposition 2}: $C^*$ is non-decreasing in $h$.\\ %\textit{Proof.} 
See appendix \ref{sec:apprendix_proofs} for a detailed mathematical proof. Intuitively, the proof consists of showing that an optimal policy can not exhibit the pathology mentioned above. Given an optimal policy $\pi^*(a|s, g, h)$ for a fixed horizon $h$ we construct a policy $\tilde \pi$ for $h+1$ which always performs better, and lower bounds the performance of $\pi^*(a|s, g, h+1)$. %\qed

In addition to being an elegant theoretical property, proposition 2 suggests that there is additional structure in a $C^*$ function which mitigates the added complexity from using horizon-aware policies. Indeed, in our preliminary experiments we used a non-cumulative version of $C$-functions (see section \ref{sec:others}) and obtained significantly improved performance upon changing to $C$-functions. Moreover, monotonicity in $h$ could be encoded in the architecture of $C^*$ \citep{sill1998monotonic, wehenkel2019unconstrained}. However, we found that actively doing so hurt empirical performance (appendix \ref{app:exp}).

\subsection{Shortcomings of $Q$-learning}
Before describing our method for learning $C^*$, we highlight a shortcoming of $Q$-learning. Consider a 2D navigation environment where an agent can move deterministically in the cardinal directions, and fix $s$ and $g$.
For an optimal action $a^*$, the optimal $Q$ function %which we are attempting to learn 
will achieve some value $Q^*(s, g, a^*) \in [0, 1]$ in the sparse reward setting. Taking a sub-optimal action $a^-$ initially results in the agent taking two extra steps to reach the intended goal, given that the agent acts optimally after the first action, so that $Q^*(s, g, a^-) = \gamma^2 Q^*(s, g, a^*)$. The value of $\gamma$ is typically chosen close to $1$, for example $0.99$, to ensure that future rewards are not too heavily discounted. As a consequence $\gamma^2 \approx 1$ and thus the value of $Q^*$ at the optimal action is very close to its value at a sub-optimal action. We illustrate this issue in Figure \ref{fig:q_accuracy}. In this scenario, recovering an optimal policy requires that the error between the learned $Q$-function and $Q^*$ should be at most $(1 - \gamma^2) / 2$; this is reflected empirically by $Q$-learning having high sample complexity and learning sub-optimal paths. This shortcoming surfaces in any environment where taking a sub-optimal action results in a slightly longer path than an optimal one, as in e.g.\ motion planning tasks.
%as is the case in motion planning tasks.


The $C^*$ function does not have this shortcoming. Consider the same 2D navigation example, and let $h^*$ be the smallest horizon for which $g$ can be reached from $s$. $h^*$ can be easily obtained from $C^*$ as
the smallest $h$ such that $\max_a C^* (s, a, g, h) = 1$.
%its first transition from $0$ to $1$.
Again, denoting $a^*$ as an optimal action and $a^-$ as a sub-optimal one, we have that $C^*(s,a^*,g,h^*) = 1$ whereas $C^*(s, a^-, g, h^*)=0$, which is illustrated in Figure \ref{fig:q_accuracy}. Therefore, the threshold for error is much higher when learning the $C^*$ function. This property results in fewer interactions with the environment needed to learn $C^*$ and more efficient solutions.

\subsection{Horizon-independent policies}
Given a $C^*$-function, equation \ref{eq:c_policy} lets us recover a horizon-aware policy. At test time, using small values of $h$ can achieve goals faster, while large values of $h$ will result in safe policies. However, a natural question arises: how small is small and how large is large? In this section we develop a method to quantitatively recover reasonable values of $h$ which adequately balance the speed/reliability trade-off. First, a safety threshold $\alpha \in (0,1]$ is chosen, which indicates the percentage of the maximum value of $C^*$ we are willing to accept as safe enough. Smaller values of $\alpha$ will thus result in quicker policies, while larger values will result in safer ones. Then we consider a range of viable horizons, $\mathcal{H}$, and find the maximal $C^*$ value, $M(s,g)=\max_{h \in \mathcal{H}, a \in \mathcal{A}} C^*(s,a,g,h)$. We then compute:
\begin{equation}
h_\alpha(s,g)=\argmin_{h \in \mathcal{H}}\{\max_{a\in\mathcal{A}}C^*(s,a,g,h) : \max_{a\in\mathcal{A}}C^*(s,a,g,h) \geq \alpha M(s,g) \},
\end{equation}
and take $\pi^*_\alpha(a|s,g) = \mathds{1}\left(a = \argmax_{a'}C^*(s, a', g, h_\alpha(s, g))\right)$. This procedure also allows us to recover horizon-independent policies from $C^*$ by using a fixed value of $\alpha$, which makes comparing against horizon-unaware methods straightforward. We used horizon-unaware policies with added randomness as the behaviour policy when interacting with the environment for exploration.


\subsection{Alternative recursions}\label{sec:others}
 One could consider defining a non-cumulative version of the $C$-function, which we call an $A$-function for ``accessibility" (\emph{not} for ``advantage''), yielding the probability of reaching a goal in exactly $h$ steps. However, this version is more susceptible to pathological behaviors that hinder learning for certain environments. For illustration, consider an agent that must move one step at a time in the cardinal directions on a checkerboard. Starting on a dark square, the probability of reaching a light square in an even number of steps is always zero, but may be non-zero for odd numbers. An optimal $A$-function would fluctuate wildly as the step horizon $h$ is increased, resulting in a harder target to learn. Nonetheless, $A$-functions admit a similar recursion to \eqref{eq:c_learning_opt}, which we include in appendix \ref{app:a_func} for completeness. In any case, the $C$-function provides a notion of reachability which is more closely tied to related work \citep{savinov2018episodic,venkattaramanujam2019self, ghosh2018learning, bharadhwaj2020leaf}.
 
 In $Q$-learning, discount factors close to $1$ encourage safe policies, while discount factors close to $0$ encourage fast policies. One could then also consider discount-conditioned policies $\pi(a|s,g,\gamma)$ as a way to achieve horizon-awareness. In appendix \ref{app:discount} we introduce $D$-functions (for ``discount''), $D(s,a,g,\gamma)$, which allow recovery of discount-conditioned policies. However $D$-functions suffer from the same limitation as $Q$-functions in that they need to be learned to a high degree of accuracy.

==> ac_learning_paper_ICLR(2)/4-method.tex <==
\section{Cumulative accessibility estimation}\label{sec:c_learning}

Our training algorithm, which we call cumulative accessibility estimation (CAE), or $C$-learning, is detailed in algorithm 1. Similarly to $Q$-learning, the $C^*$ function can be modelled as a neural network with parameters $\theta$, denoted $C^*_\theta$, which can be learned by minimizing:
\begin{equation}
\label{eq:loss_fn}
-\sum_i \left[y_i \log C^*_\theta(s_i,a_i,g_i,h_i) + (1-y_i)\log \left(1 - C^*_\theta(s_i,a_i,g_i,h_i)\right) \right],
\end{equation}
where $y_i$ corresponds to a stochastic estimate of the right hand side of equation \ref{eq:c_learning_opt}.
The sum is over tuples $(s_i, a_i, s'_{i}, g_i, h_i)$ drawn from a replay buffer which we specially tailor to successfully learn $C^*$. Since $C^*$ corresponds to a probability, we change the usual squared loss to be the binary cross entropy loss. Note that even if the targets $y_i$ are not necessarily binary, the use of binary cross entropy is still justified as it is equivalent to minimizing the $\mathbb{KL}$ divergence between Bernoulli distributions with parameters $y_i$ and $C_\theta^*(s_i, a_i, g_i, h_i)$ \citep{bellemare2017distributional}. 
Since the targets used do not correspond to the right-hand side of equation \ref{eq:c_learning_opt} but to a stochastic estimate (through $s_i'$) of it, using this loss instead of the square loss results in an \emph{unbiased} estimate of $\sum_i \mathcal{L}(C_\theta^*(s_i,a_i,g_i,h_i), y_i^{\mathrm{true}})$, where $y_i^{\mathrm{true}}$ corresponds to the right-hand side of equation \ref{eq:c_learning_opt} at $(s_i, a_i, g_i, h_i)$ (see appendix \ref{app:ce} for a detailed explanation). This confers another benefit of $C$-learning over $Q$-learning, as passing a stochastic estimate of equation \ref{eq:q_learning} through the typical squared loss results in \emph{biased} estimators.
As in Double $Q$-learning \citep{van2015deep}, we use a second network $C^*_{\theta^{\prime}}$ to compute the $y_i$ targets, and do not minimize equation \ref{eq:loss_fn} with respect to $\theta^{\prime}$. We periodically update $\theta^{\prime}$ to match $\theta$. We now explain our algorithmic details.

\textbf{Reachability-guided sampling}: When sampling a batch (line \ref{alg_line:sample_batch} of algorithm 1), for each $i$ we first sample an episode from $\mathcal{D}$, and then a transition $(s_i, a_i, s^{\prime}_i)$ from that episode. We sample $h_i$ favoring smaller $h$'s at the beginning of training. We achieve this by selecting $h_i=h$ with probability proportional to $h^{-\kappa n_{GD} / N_{GD}}$, where $n_{GD}$ is the current episode number, $N_{GD}$ the total number of episodes, and $\kappa$ is a hyperparameter. For deterministic environments, we follow HER \citep{andrychowicz2017hindsight} and select $g_i$ uniformly at random from the states observed in the episode after $s_i$. For stochastic environments we use a slightly modified version, which addresses the bias incurred by HER \citep{multigoal} in the presence of stochasticity. All details are included in appendix \ref{app:exp1}.

\textbf{Extension to continuous action spaces}: Note that constructing the targets $y_i$ requires taking a maximum over the action space. While this is straightforward in discrete action spaces, it is not so for continuous actions. \citet{lillicrap2015continuous} proposed DDPG, a method enabling deep $Q$-learning in continuous action spaces. Similarly, \citet{fujimoto2018addressing} proposed TD3, a method for further stabilizing $Q$-learning. We note that $C$-learning is compatible with the ideas underpinning both of these methods. We present a TD3 version of $C$-learning in appendix \ref{app:cont}. 

\begin{algorithm}[!t]
\label{algo:C-learning}
    \DontPrintSemicolon
    \SetKwFor{RepTimes}{repeat}{times}{}
    \caption{Training C-learning Network}
    \SetKwInOut{Parameter}{Parameter}
    \Parameter{$N_{\mathrm{explore}}$: Number of random exploration episodes}
    \Parameter{$N_{\mathrm{GD}}$: Number of goal-directed episodes}
    \Parameter{$N_{\mathrm{train}}$: Number of batches to train on per goal-directed episode}
    \Parameter{$N_{\mathrm{copy}}$: Number of batches between target network updates}
    \Parameter{$\alpha$: Learning rate}
    $\theta \gets$ Initial weights for $C^*_\theta$ \;
    $\theta^{\prime} \gets \theta$ \tcp*{Copy weights to target network}
    $\mathcal{D} \gets$\texttt{[]} \tcp*{Initialize experience replay buffer}
    %Dataset to hold rollout history
    $n_{\mathrm{b}} \gets 0$ \tcp*{Counter for training batches}
    \RepTimes{$N_{\mathrm{explore}}$}{
        $\mathcal{E} \gets \mathtt{get\_rollout(}\pi_{\mathrm{random}}\mathtt{)} $ \tcp*{Do a random rollout}
        $\mathcal{D}\mathtt{.append(}\mathcal{E}\mathtt{)}$ \tcp*{Save the rollout to the buffer}
    }
    \RepTimes{$N_{\mathrm{GD}}$}{
        $g \gets \mathtt{goal\_sample(}\mathcal{}  n_{\mathrm{b}}\mathtt{)}$ \tcp*{Sample a goal}\label{alg_line:goal_sample}
        $\mathcal{E} \gets \mathtt{get\_rollout(}\pi_{\mathrm{behavior}}\mathtt{)} $ \tcp*{Try to reach the goal}\label{alg_line:get_rollout}
        $\mathcal{D}\mathtt{.append(}\mathcal{E}\mathtt{)}$ \tcp*{Save the rollout}
        \RepTimes{$N_{\mathrm{train}}$}{
            \uIf{$n_{\mathrm{b}} \mod N_{\mathrm{copy}} = 0$}{
                $\theta^{\prime} \gets \theta$ \tcp*{Copy weights periodically}
            }
            $\mathcal{B}:=\{s_i, a_i, s'_i, g_i, h_i\}_{i=1}^{|\mathcal{B}|}\gets \mathtt{sample\_batch(}\mathcal{D}\mathtt{)}$ \tcp*{Sample a batch}\label{alg_line:sample_batch}
            $\left\{y_i\right\}_{i=1}^{\left| \mathcal{B} \right|} \gets \mathtt{get\_targets(}\mathcal{B}, \theta^{\prime}\mathtt{)}$ \tcp*{Estimate RHS of equation \ref{eq:c_learning_opt}}\label{alg_line:get_targets}
            $\hat{\mathcal{L}} \gets -\frac{1}{\left| \mathcal{B} \right|} \sum_{i=1}^{\left|\mathcal{B}\right|} y_i \log C^*_\theta(s_i,a_i,g_i,h_i) + (1-y_i)\log \left(1 - C^*_\theta(s_i,a_i,g_i,h_i)\right)$ \;
            $\theta \gets \theta - \alpha \nabla_\theta \hat{\mathcal{L}}$  \tcp*{Update weights}
            $n_{\mathrm{b}} \gets n_{\mathrm{b}} + 1$ \tcp*{Trained one batch}
        }
    }
\end{algorithm}

We finish this section by highlighting differences between $C$-learning and related work. \citet{Ghosh2019} proposed GCSL, a method for goal-reaching inspired by supervised learning. In their derivations, they also include a horizon $h$ which their policies can depend on, but they drop this dependence in their experiments as they did not see a practical benefit by including $h$. We find the opposite for $C$-learning. TDMs \citep{pong2018temporal} use horizon-aware policies and a similar recursion to ours. In practice they use a negative $L_1$ distance reward, which significantly differs from our goal-reaching indicators. This is an important difference as TDMs operate under dense rewards, while we use sparse rewards, making the problem significantly more challenging. Additionally, distance between states in nonholonomic environments is very poorly described by $L_1$ distance, resulting in TDMs being ill-suited for motion planning tasks. We also highlight that even if the reward in TDMs was swapped with our goal checking function $G$, the resulting objective would be much closer to the non-cumulative version of $C$-learning presented in appendix \ref{app:a_func}. TDMs recover policies from their horizon-aware $Q$-function in a different manner to ours, not allowing a speed vs reliability trade-off. The recursion presented for TDMs is used by definition, whereas we have provided a mathematical derivation of the Bellman equation for $C$-functions along with proofs of additional structure. As a result of the $C$-function being a probability we use a different loss function (binary cross-entropy) which results in unbiased estimates of the objective's gradients. Finally, we point out that TDMs sample horizons uniformly at random, which differs from our specifically tailored replay buffer.

==> ac_learning_paper_ICLR(2)/5-experiments.tex <==
\section{Experiments}\label{sec:experiments}

% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}[t]{.3\linewidth}
%     %\caption{Frozen lake}
%     \includegraphics[scale=0.35]{figures/frozen_lake.png}
%     \end{subfigure}
%     \begin{subfigure}[t]{.3\linewidth}
%     %\caption{Mini maze}
%     \includegraphics[scale=0.35]{figures/mini_maze.png}
%     \end{subfigure}
%     \begin{subfigure}[t]{.3\linewidth}
%     %\caption{Dubins' car}
%     \includegraphics[scale=0.349]{figures/dubins_car.png}
%     \end{subfigure}
%     \caption{Experimental environments: frozen lake (left), mini maze (middle), and Dubins car (right). Arrows represent actions (only their direction should be considered, their magnitude is not representative of the distance travelled by an agent taking an action). See text for description.}
%     \label{fig:envs}
% \end{figure}

% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}[t]{.245\linewidth}
%     \centering
%     %\caption{Frozen lake}
%     \includegraphics[scale=0.58]{figures/frozen_lake.png}
%     \end{subfigure}
%     \begin{subfigure}[t]{.245\linewidth}
%     \centering
%     \includegraphics[scale=0.58]{figures/dubins_car.png}
%     \end{subfigure}
%     \begin{subfigure}[t]{.245\linewidth}
%     \centering
%     \includegraphics[scale=0.29]{figures/pick.png}
%     \end{subfigure}
%     \begin{subfigure}[t]{.245\linewidth}
%     \centering
%     \includegraphics[scale=0.29]{figures/pen.png}
%     \end{subfigure}
%     \caption{Experimental environments: frozen lake (first), Dubins' car (second), FetchPickAndPlace-v1 (third) and HandManipulatePenFull-v0 (fourth). Arrows represent actions (only their direction should be considered, their magnitude is not representative of the distance travelled by an agent taking an action). See text for description.}
%     \label{fig:envs}
% \end{figure}

\subsection{Setup}

Our experiments are designed to show that $(i)$ $C$-learning enables the speed vs reliability trade-off, $(ii)$ the $C^*$ function recovered through $C$-learning meaningfully matches reachability in nonholonomic environments, and $(iii)$ $C$-learning scales to complex and high-dimensional motion planning tasks, resulting in improved sample complexity and goal-reaching. We use success rate (percentage of trajectories which reach the goal) and path length (average, over trajectories and goals, number of steps needed to achieve the goal among successful trajectories) as metrics.

We compare $C$-learning against GCSL \citep{Ghosh2019} (for discrete action states only) and deep $Q$-learning with HER \citep{andrychowicz2017hindsight} across several environments, which are depicted in Figure \ref{fig:envs}. All experimental details and hyperparameters are given in appendix \ref{app:exp1}. We also provide ablations, and comparisons against TDMs and the alternative recursions from section \ref{sec:others} in appendix \ref{app:exp}. We evaluate $C$-learning on the following domains:
\begin{enumerate}[
    topsep=0pt,
    noitemsep,
    partopsep=0.5ex,
    parsep=0.5ex,
    leftmargin=*,
    itemindent=2.5ex
    ]
\item \textbf{Frozen lake} is a 2D  navigation environment where the agent must navigate without falling in the holes (dark blue). Both the state space ($7 \times 5$ grid, with two $3 \times 1$ holes) and the action state are discrete. Falling in a hole terminates an episode. The agent's actions correspond to intended directions. The agent moves in the intended direction with probability $0.8$, and in perpendicular directions with probabilities $0.1$ each. %(the agent never moves in the exact opposite direction as the intended one). 
Moving against the boundaries of the environment has no effect. We take $\mathcal{G} = \mathcal{S}$ and $G(s, g)=\mathds{1}(g=s)$.

% \item \textbf{Mini maze} is a deterministic 2D navigation environment, where moving against the boundaries or the walls has no effect. Actions and states ($24 \times 24$ grid) are discrete, and goals also match states.

\item \textbf{Dubins' car} is a more challenging deterministic 2D navigation environment, where the agent drives a car which cannot turn by more than $10^{\circ}$. The states, with spatial coordinates in $[0,15]^2$, are continuous and include the direction of the car. There are 7 actions: the $6$ combinations of $\left\{\mathrm{left}\,10^{\circ},\, \mathrm{straight},\, \mathrm{right}\,10^{\circ}\right\} \times \left\{\mathrm{forward\,1},\, \mathrm{reverse\,1}\right\}$, and the option to not move.
As such, the set of reachable states is not simply a ball around the current state. The environment also has walls through which the car cannot drive.
We take $\mathcal{G}=[0,15]^2$ and the goal is considered to be reached when the car is within an $L_\infty$ distance of $0.5$ from the goal, regardless of its orientation.
%States are continuous, and we take goals to correspond to the spatial coordinates of states, while reaching a goal is defined as the state's spatial coordinates being within an $L_2$ ball of radius $0.5$ around the goal.

% \item \textbf{Reacher} is a robotic arm control environment where the agent needs to maneuver the tip of the arm to the target location. We use the hard version of reacher. Actions are continuous and control the joints of the arm, while states correspond to angles of the joints and their momentum. Reaching a goal is defined as being within an $L_2$ distance of $0.025$ of the goal. Since there is no natural metric $d$ for reachability-guided sampling or $C$-function clipping, we simply sample goals uniformly at random, thus using a simplified version of our replay buffer. We found that $C$-learning still performed excellently even in this setting, probably due to the fact that a goals occupy a relatively large volume of the space (which is $0.4 \times 0.4$) as compared to other environments.
\item \textbf{FetchPickAndPlace-v1} \citep{openAIgym} is a complex, higher-dimensional environment in which a robotic arm needs to pick up a block and move it to the goal location. Goals are defined by their 3-dimensional coordinates. The state space is $25$-dimensional, and the action space is continuous and $4$-dimensional.

\item \textbf{HandManipulatePenFull-v0} \citep{openAIgym} is a realistic environment known the be a difficult goal-reaching problem, where deep Q-learning with HER shows very limited success \citep{plappert2018multi}. The environment has a continuous action space of dimension $20$, a $63$-dimensional state space, and $7$-dimensional goals. Note that we are considering the more challenging version of the environment where both target location and orientation are chosen randomly.
\end{enumerate}

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.6]{figures/frozen_lake.png}
    \includegraphics[scale=0.6]{figures/dubins_car.png}
    \includegraphics[scale=0.3]{figures/pick.png}
    \includegraphics[scale=0.3]{figures/pen.png}
    \caption{Experimental environments, from left to right: frozen lake, Dubins' car, FetchPickAndPlace-v1 and HandManipulatePenFull-v0. Arrows represent actions (only their direction should be considered, their magnitude is not representative of the distance travelled by an agent taking an action). See text for description.}
    \label{fig:envs}
\end{figure}

\subsection{Results}

\textbf{Speed vs reliability trade-off}: We use frozen lake to illustrate this trade-off. At test time, we set the starting state and goal as shown in Figure \ref{fig:frozen_lake}. Notice that, given enough time, an agent can reach the goal with near certainty by going around the holes on the right side of the lake. However, if the agent is time-constrained, the optimal policy must accept the risk of falling in a hole.
We see that $C$-learning does indeed learn both the risky and safe policies.
Other methods, as previously explained, can only learn one.
%Note that plotting all the values from our $C$-learning policy would require plotting the environment once for every considered value of $h$, so that instead the arrows on Figure \ref{fig:frozen_lake} correspond to $\argmax_{a} \pi^*(a|s,g,h)$, $\argmax_{a} \pi^*(a|s_1,g,h-1)$, $\argmax_{a} \pi^*(a|s_2,g,h-2)$ and so on,  where $s_{t+1}$ is obtained from the previous state and action while ignoring the randomness in the environment (i.e. $s_{t+1} = \argmax_s p(s|s_t, a_t)$).
To avoid re-plotting the environment for every horizon, we have plotted arrows in Figure \ref{fig:frozen_lake} corresponding to $\argmax_{a} \pi^*(a|s_0,g,h)$, $\argmax_{a} \pi^*(a|s_1,g,h-1)$, $\argmax_{a} \pi^*(a|s_2,g,h-2)$ and so on,  where $s_{t+1}$ is obtained from the previous state and action while ignoring the randomness in the environment (i.e. $s_{t+1} = \argmax_s p(s|s_t, a_t)$).
In other words, we are plotting the most likely trajectory of the agent.
When given the minimal amount of time to reach the goal ($h=6$), the CAE agent learns correctly to accept the risk of falling in a hole by taking the direct path. When given four times as long ($h=24$), the agent takes a safer path by going around the hole. Notice that the agent makes a single mistake at the upper right corner, which is quickly corrected when the value of $h$ is decreased. On the other hand, we can see on the bottom panel that both GCSL and HER recover a single policy, thus not enabling the speed vs reliability trade-off.
%Surprisingly, GCSL learns to always go up, when it should learn to go around the holes since there is nothing in its objective function encouraging reaching the goal quickly.
Surprisingly, GCSL learns to take the high-risk path, despite \citet{Ghosh2019}'s intention to incentivize paths that are guaranteed to reach the goal.

% \begin{figure}[!t]
%     \centering
%     \includegraphics[scale=0.4]{figures/frozen_lake_tradeoff.png}
%     \includegraphics[scale=0.4]{figures/frozen_lake_her.png}
%     \caption{Policies recovered by $C$-learning in frozen lake for different values of $h$ for reaching $(G)$ from $(S)$ (left); and policies recovered by GCSL and HER (right).}
%     \label{fig:frozen_lake}
% \end{figure}

% \begin{figure}[!t]
% \centering
% %\vspace{-0.3cm}
% \begin{minipage}[b]{.65\linewidth}
%     \centering
%     \includegraphics[width=0.49\textwidth]{figures/frozen_lake_tradeoff.png}
%     \includegraphics[width=0.49\textwidth]{figures/frozen_lake_her.png}
% \end{minipage}
% \begin{minipage}[b]{.34\linewidth}
%     \centering
%     \caption{Multimodal policies recovered by $C$-learning in frozen lake for different values of $h$ for reaching $(G)$ from $(S)$ (left); unimodal policies recovered by GCSL and HER (right).}
%     \label{fig:frozen_lake}
% \end{minipage}
% \end{figure}

\textbf{Reachability learning}: To demonstrate that we are adequately learning reachability, we removed the walls from Dubins' car and further restricted the turning angles to $5^\circ$, thus making the dumbbell shape of the true reachable region more extreme. In Figure \ref{fig:reachability}, we show that our learned $C^*$ function correctly learns which goals are reachable from which states for different time horizons in Dubins' car:
not only is the learned $C^*$ function increasing in $h$, but the shapes are as expected.
None of the competing alternatives recover this information in any way, and thus comparisons are not available. As previously mentioned, the optimal $C^*$-function in this task is not trivial.
Reachability is defined by the ``geodesics'' in $\mathcal{S} = \left[0, 15\right]^2 \times S^1$ that are constrained by the finite turning radius, and thus follow a more intricate structure than a ball in $\mathbb{R}^2$.

% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}[t]{.245\linewidth}
%     \centering
%     %\caption{Frozen lake}
%     \includegraphics[scale=0.58]{figures/frozen_lake.png}
%     \end{subfigure}
%     \begin{subfigure}[t]{.245\linewidth}
%     \centering
%     \includegraphics[scale=0.58]{figures/dubins_car.png}
%     \end{subfigure}
%     \begin{subfigure}[t]{.245\linewidth}
%     \centering
%     \includegraphics[scale=0.29]{figures/pick.png}
%     \end{subfigure}
%     \begin{subfigure}[t]{.245\linewidth}
%     \centering
%     \includegraphics[scale=0.29]{figures/pen.png}
%     \end{subfigure}
%     \caption{Experimental environments: frozen lake (first), Dubins' car (second), FetchPickAndPlace-v1 (third) and HandManipulatePenFull-v0 (fourth). Arrows represent actions (only their direction should be considered, their magnitude is not representative of the distance travelled by an agent taking an action). See text for description.}
%     \label{fig:envs}
% \end{figure}

\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[scale=0.39, trim={5cm 0 5cm 0}]{figures/frozen_lake_tradeoff.png}\\
        \includegraphics[scale=0.39, trim={5cm 0 5cm 0}]{figures/frozen_lake_her.png}
        \caption{}
        \label{fig:frozen_lake}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[scale=0.365]{figures/dubin_7.png}\\
        \includegraphics[scale=0.365]{figures/dubin_15.png}\\
        \includegraphics[scale=0.365]{figures/dubin_25.png}
        \caption{}
        \label{fig:reachability}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[scale=0.162]{figures/traj_c_learning.png}\\
        \includegraphics[scale=0.162]{figures/traj_gcsl.png}\\
        \includegraphics[scale=0.162]{figures/traj_her.png}
        \caption{}
        \label{fig:dubins}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[trim=40 8 30 25, clip,width=1.04\textwidth]{figures/Dubins_curves.png}\\
        \includegraphics[trim=32 8 30 25, clip,width=1.04\textwidth]{figures/pick_curve.png}\\
        \includegraphics[trim=42 8 30 25, clip,width=1.04\textwidth]{figures/hand_curves.png}
        \caption{}
        \label{fig:training_plots}
    \end{subfigure}
    \caption{$(a)$ Multimodal policies recovered by $C$-learning in frozen lake for different values of $h$ for reaching $(G)$ from $(S)$ (top); unimodal policies recovered by GCSL and HER (bottom). $(b)$ Heatmaps over the goal space of $\max_{a} C^*(s,a,g,h)$ with a fixed $s$ and $h$ for Dubins' car, with $h=7$ (top), $h=15$ (middle) and $h=25$ (bottom). $(c)$ Trajectories learned by $C$-learning (top), GCSL (middle) and HER (bottom) for Dubins' car. $(d)$ Success rate throughout the training for Dubins' car (top), FetchPickAndPlace-v1 (middle) and HandManipulatePenFull-v0 (bottom) for $C$-learning (blue), HER (red) and GCSL (green).}
\end{figure}

% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}[b]{0.3\textwidth}
%     \includegraphics[scale=0.5]{figures/dubin_7.png}
%     \caption{$h=7$}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.3\textwidth}
%     \includegraphics[scale=0.5]{figures/dubin_15.png}
%     \caption{$h=15$}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.3\textwidth}
%     \includegraphics[scale=0.5]{figures/dubin_25.png}
%     \caption{$h=25$}
%     \end{subfigure}
%     \caption{Heatmaps over the goal space of $\max_{a} C^*(s,a,g,h)$ with a fixed $s$ and $h$ for Dubins' car.}
%     \label{fig:reachability}
% \end{figure}

\textbf{Motion planning and goal-reaching}: For a qualitative comparison of performance for goal-reaching, Figure \ref{fig:dubins} shows trajectories for $C$-learning and competing alternatives for Dubins' car. We can see that $C$-learning finds the optimal route, which is a combination of forward and backward movement, while other methods find inefficient paths. We also evaluated our method on challenging goal reaching environments, and observed that $C$-learning achieves state-of-the-art results both in sample complexity and success rate. Figure \ref{fig:training_plots} shows that $C$-learning is able to learn considerably faster in the FetchPickAndPlace-v1 environment. More importantly, $C$-learning achieves an absolute $20\%$ improvement in its success rate over the current state-of-the-art algorithm HER (TD3) in the HandManipulatePenFull-v0 environment. Quantitative results are shown in Table \ref{tab:results}.
On Dubins' car, we also note that $C$-learning ends up with a smaller final $L_\infty$ distance to the goal: $\mathbf{0.93 \pm 0.15}$ vs.\ $1.28 \pm 0.51$ for GCSL.

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.2]{figures/traj_c_learning.png}
%     \includegraphics[scale=0.2]{figures/traj_gcsl.png}
%     \includegraphics[scale=0.2]{figures/traj_her.png}
%     \caption{Trajectories learned by $C$-learning (left), GCSL (middle) and HER (right).}
%     \label{fig:dubins}
% \end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.23\textwidth}
%     \centering
%     \includegraphics[trim=16 8 30 25, clip, width=1.\textwidth]{figures/Precipice_curves.png}
%     \caption{}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[b]{0.23\textwidth}
%     \centering
%     \includegraphics[trim=16 8 30 25, clip,width=1.\textwidth]{figures/Dubins_curves.png}
%     \caption{}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[b]{0.23\textwidth}
%     \centering
%     \includegraphics[trim=16 8 30 25, clip,width=1.\textwidth]{figures/pick_curve.png}
%     \caption{}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[b]{0.23\textwidth}
%     \centering
%     \includegraphics[trim=16 8 30 25, clip,width=1.\textwidth]{figures/hand_curves.png}
%     \caption{}
%     \end{subfigure}
%     \caption{Success rate throughout the training for $(a)$ frozen lake, $(b)$ Dubins' car, $(c)$ FetchPickAndPlace-v1 and $(d)$ HandManipulatePenFull-v0.}
%     \label{fig:training_plots}
% \end{figure}

% \begin{table}[h]
% \footnotesize
% \caption{Relevant metrics for goal-reaching, stratified by difficulty of goal. Runs in \textbf{bold} are either the best on the given metric for the given environment, or have overlapping error bars with the best.}
% \centering
% \resizebox{0.8\textwidth}{!}{  
% \begin{tabular}{c|c|cccc|cccc}
%     \toprule
%     \multirow{2}{*}{\textbf{ENV}}& \multirow{2}{*}{\textbf{METHOD}} & \multicolumn{4}{c}{\textbf{FINAL DISTANCE}} & \multicolumn{4}{c}{\textbf{TRAVELLED DISTANCE}}\\
%      &  & EASY & MED & HARD & \textbf{ALL}  & EASY & MED & HARD & \textbf{ALL}\\
%     \hline
%     %\multicolumn{2}{c}{\multirow{2}{*}{Multi-col-row}}&X\\
%     \multirow{3}{*}{Frozen lake} & CAE & -- & -- & -- & $\mathbf{1.39}$ & -- & -- & -- & $\mathbf{5.57}$\\
%      & GCSL & -- & -- & -- & $\mathbf{1.34}$ & -- & -- & -- & $\mathbf{5.47}$\\
%      & HER & -- & -- & -- & $2.71$ & -- & -- & -- & $\mathbf{6.42}$\\
%      \hline
%      \multirow{3}{*}{Mini maze} & CAE & $\mathbf{0.00}$ & $\mathbf{0.58}$ & $11.69$ & $3.22$ & $\mathbf{5.70}$ & $\mathbf{27.41}$ & $\mathbf{18.03}$ & $\mathbf{19.67}$\\
%      & GCSL & $0.44$ & $1.29$ & $\mathbf{5.10}$ & $\mathbf{2.03}$ & $20.08$ & $\mathbf{24.66}$ & $\mathbf{18.50}$ & $\mathbf{21.97}$\\
%      & HER & $5.16$ & $3.02$ & $7.91$ & $4.77$ & $81.27$ & $111.62$ & $\mathbf{18.28}$ & $80.70$\\
%      \hline
%      \multirow{3}{*}{Dubins' car} & CAE & $2.09$ & $\mathbf{2.78}$ & $\mathbf{0.91}$ & $\mathbf{1.78}$ & $\mathbf{9.05}$ & $\mathbf{30.02}$ & $\mathbf{20.79}$ & $\mathbf{21.53}$\\
%      & GCSL & $\mathbf{0.33}$ & $\mathbf{2.28}$ & $5.63$ & $3.42$ & $\mathbf{8.06}$ & $61.31$ & $87.77$ & $62.63$\\
%      & HER & $5.05$ & $6.94$ & $7.60$ & $6.86$ & $51.98$ & $57.57$ & $64.87$ & $59.78$\\
%      \bottomrule
% \end{tabular}
% }
% \label{tab:results}
% \end{table}

\begin{table}[!t]
\caption{Comparison of $C$-Learning against relevant benchmarks in three environments, averaged across five random seeds.
Runs in \textbf{bold} are either the best on the given metric in that environment, or have a mean score within the error bars of the best.}
\centering
\resizebox{0.85\textwidth}{!}{  
\begin{tabular}{c|c|c|c}
    \toprule
    \multirow{2}{*}{\textbf{ENVIRONMENT}}& \multirow{2}{*}{\textbf{METHOD}} &
    \multirow{2}{*}{\textbf{SUCCESS RATE}}&
    \multirow{2}{*}{\textbf{PATH LENGTH}}\\
    \\
    \hline
    %\multicolumn{2}{c}{\multirow{2}{*}{Multi-col-row}}&X\\
    
    % \rowcolor{vvlightgray}
    % \multirow{3}{*}{\cellcolor{white}Frozen lake} & CAE & -- & $\mathbf{1.54}$ & $\mathbf{5.14}$\\
    %  & GCSL & -- & $\mathbf{1.50}$ &  $\mathbf{7.18}$\\
    %  & HER & -- &  $\mathbf{2.01}$ & $\mathbf{6.58}$\\
    %  \hline
     
     \rowcolor{vvlightgray}
     \multirow{3}{*}{\cellcolor{white}Dubins' Car} & CAE & $\mathbf{86.15\% \pm 2.44} \%$ & $\mathbf{16.45 \pm 0.99}$ \\%& $\mathbf{0.70}$  \\
     & GCSL & $79.69\% \pm 6.35\%$ & $32.64 \pm 6.16$ \\%& $1.28 \pm 0.51$ \\
     & HER & $51.25\% \pm 6.48\%$ & $20.13 \pm 1.66$ \\%& $4.03 \pm 1.04$ \\
    %  & HER & $5.16$ & $3.02$ & $7.91$ & $4.77$ & $81.27$ & $111.62$ & $\mathbf{18.28}$ & $80.70$\\
     \hline
     \rowcolor{vvlightgray}
     \multirow{2}{*}{\cellcolor{white}FetchPickAndPlace-v1} & CAE (TD3)& $\mathbf{99.34\% \pm 0.27\%}$  & $\mathbf{8.53\pm 0.09}$\\% & --\\
     & HER (TD3)& $98.25\% \pm 2.51\%$ & $8.86 \pm 0.14$\\% &  --\\
       \hline
     \rowcolor{vvlightgray}
     \multirow{2}{*}{\cellcolor{white}HandManipulatePenFull-v0} & CAE (TD3) & $\mathbf{39.83\% \pm 1.64\%}$ & $\mathbf{7.68 \pm 0.90}$\\%  & --\\
     & HER (TD3)& $21.99\% \pm 2.46\%$ & $15.03 \pm 0.71$\\% & --\\
     \bottomrule
\end{tabular}
}
\label{tab:results}
\end{table}



==> ac_learning_paper_ICLR(2)/6-disc.tex <==

\section{Discussion}

We have shown that $C$-learning enables simultaneous learning of how to reach goals quickly and how to reach them safely, which current methods cannot do. We point out that reaching the goal safely in our setting means doing so at test time, and is different to what is usually considered in the safety literature where safe exploration is desired \citep{chow2018lyapunov, bharadhwaj2020conservative}. Additionally, learning $C^*$ effectively learns reachability within an environment, and could thus naturally lends itself to incorporation into other frameworks, for example, in goal setting for hierarchical RL tasks \citep{nachum2018data} where intermediate, reachable goals need to be selected sequentially. We believe further investigations on using $C$-functions on safety-critical environments requiring adaptation \citep{peng2018sim, zhang2020carl}, or for hierarchical RL, are promising directions for further research. 

We have also argued that $C$-functions are more tolerant of errors during learning than $Q$-functions which increases sample efficiency. This is verified empirically in that $C$-learning is able to solve goal-reaching tasks earlier on in training than $Q$-learning.

We finish by noticing a parallel between $C$-learning and the options framework \citep{sutton1999between, bacon2017option}, which introduces temporal abstraction and allows agents to not always follow the same policy when at a given state $s$. However, our work does not fit within this framework, as options evolve stochastically and new options are selected according only to the current state, while horizons evolve deterministically and depend on the previous horizon only, not the state. Additionally, and unlike $C$-learning, nothing encourages different options to learn safe or quick policies, and there is no reachability information contained in options.




==> ac_learning_paper_ICLR(2)/7-conc.tex <==
\section{Conclusions}\label{sec:conclusions}

In this paper we introduced $C$-learning, a $Q$-learning-inspired method for goal-reaching. Unlike previous approaches, we propose the use of horizon-aware policies, and show that not only can these policies be tuned to reach the goal faster or more reliably, but they also outperform horizon-unaware approaches for goal-reaching on complex motion planning tasks. We hope our method will inspire further research into horizon-aware policies and their benefits.
